Commonsense Properties from Query Logs and Question Answering Forums

Commonsense knowledge about object properties, human behavior and general concepts is crucial for robust AI applications. However, automatic acquisition of this knowledge is challenging because of sparseness and bias in online sources. This paper presents Quasimodo, a methodology and tool suite for distilling commonsense properties from non-standard web sources. We devise novel ways of tapping into search-engine query logs and QA forums, and combining the resulting candidate assertions with statistical cues from encyclopedias, books and image tags in a corroboration step. Unlike prior work on commonsense knowledge bases, Quasimodo focuses on salient properties that are typically associated with certain objects or concepts. Extensive evaluations, including extrinsic use-case studies, show that Quasimodo provides better coverage than state-of-the-art baselines with comparable quality.

==> figures/source-recall-diagram.tex <==

\begin{tikzpicture}
\begin{axis}[
    ybar,
    bar width=0.2cm,
    height=5cm,
    width=\columnwidth,
    enlarge y limits=0.05,
    enlarge x limits=0.15,
    legend style={anchor=north east,legend columns=1},
    ylabel={recall (\%)},
    ylabel near ticks,
    symbolic x coords={strict,relaxed, strict$@$5, relaxed$@$5},
    xtick=data,
    ]
\addplot[black,fill=yellow,pattern=north east lines] coordinates {(relaxed,20.02) (strict, 7.55) (relaxed$@$5,6.15) (strict$@$5, 1.86)};
\addplot[olive,fill=olive] coordinates {(relaxed,11.08) (strict,9.31) (relaxed$@$5,0.92) (strict$@$5,0.85)};
\addplot[teal,fill=teal] coordinates {(relaxed,32.09) (strict,16.47) (relaxed$@$5,3.64) (strict$@$5,1.03)};
\addplot[blue,fill=blue] coordinates {(relaxed,57.84) (strict,28.10)};% (relaxed$@$5,0) (strict$@$5,0)};
\addplot[black,fill=blue!25!white] coordinates {(relaxed$@$5,10.96) (strict$@$5,8.35)};
\addplot[black,fill=blue!75!black] coordinates {(relaxed$@$5,11.16) (strict$@$5,5.22)};
\legend{ConceptNet,WebChild,TupleKB,Q'modo, Q'modo-$\tau$, Q'modo-$\sigma$}
\end{axis}
\end{tikzpicture}






% part 1: full only
\begin{tikzpicture}
\begin{axis}[
    ybar,
    bar width=0.2cm,
    height=5cm,
    width=0.5\columnwidth,
    enlarge y limits=0.05,
    enlarge x limits=0.15,
    legend style={anchor=north east,legend columns=1},
    ylabel={recall (\%)},
    ylabel near ticks,
    symbolic x coords={strict,relaxed, strict$@$5, relaxed$@$5},
    xtick=data,
    ]
\addplot[black,fill=yellow,pattern=north east lines] coordinates {(relaxed,20.02) (strict, 7.55)};
\addplot[olive,fill=olive] coordinates {(relaxed,11.08) (strict,9.31)};
\addplot[teal,fill=teal] coordinates {(relaxed,32.09) (strict,16.47)};
\addplot[blue,fill=blue] coordinates {(relaxed,57.84) (strict,28.10)};% (relaxed$@$5,0) (strict$@$5,0)};
\legend{ConceptNet,WebChild,TupleKB,Q'modo}
\end{axis}
\end{tikzpicture}
% part 2: @5 only
\begin{tikzpicture}
\begin{axis}[
    ybar,
    bar width=0.2cm,
    height=5cm,
    width=0.5\columnwidth,
    enlarge y limits=0.05,
    enlarge x limits=0.15,
    legend style={anchor=north east,legend columns=1},
    ylabel={recall (\%)},
    ylabel near ticks,
    symbolic x coords={strict,relaxed, strict$@$5, relaxed$@$5},
    xtick=data,
    ]
\addplot[black,fill=yellow,pattern=north east lines] coordinates {(relaxed$@$5,6.15) (strict$@$5, 1.86)};
\addplot[olive,fill=olive] coordinates {(relaxed$@$5,0.92) (strict$@$5,0.85)};
\addplot[teal,fill=teal] coordinates {(relaxed$@$5,3.64) (strict$@$5,1.03)};
\addplot[blue,fill=blue] coordinates { };% (relaxed$@$5,0) (strict$@$5,0)};
\addplot[black,fill=blue!25!white] coordinates {(relaxed$@$5,10.96) (strict$@$5,8.35)};
\addplot[black,fill=blue!75!black] coordinates {(relaxed$@$5,11.16) (strict$@$5,5.22)};
\legend{ConceptNet,WebChild,TupleKB,Q'modo,Q'modo-$\tau$, Q'modo-$\sigma$}
\end{axis}
\end{tikzpicture}




=================
the latest from the document!


\begin{tikzpicture}
\begin{axis}[
    ybar,
    bar width=0.15cm,
    height=3.3cm,
    width=5cm,
%    enlarge y limits=0.05,
    enlarge x limits=0.45,
%    legend style={anchor=north east,legend columns=1},
    legend style={at={(0.5,-0.6)},
    anchor=north,legend columns=1},
    ylabel={recall (\%)},
    ylabel near ticks,
    symbolic x coords={strict,relaxed, strict$@$5, relaxed$@$5},
    xtick=data,
    ]
%\addlegendimage{no markers,green}    
\addplot[black,fill=yellow,pattern=north east lines] coordinates {(relaxed,2.76) (strict, 3.10)};
\addplot[olive,fill=olive] coordinates {(relaxed,6.6) (strict,6.04)};
\addplot[teal,fill=teal] coordinates {(relaxed,31.29) (strict,16.00)};
\addplot[blue,fill=blue] coordinates {(relaxed,52.99) (strict,24.28)};% (relaxed$@$5,0) (strict$@$5,0)};
\legend{ConceptNet,WebChild,TupleKB,Q'modo}
\end{axis}
\end{tikzpicture}
% part 2: @5 only
\begin{tikzpicture}
\begin{axis}[
    ybar,
    bar width=0.15cm,
    height=3.3cm,
    enlarge x limits=0.45,
    width=5cm,
    legend style={at={(0.5,-0.6)},
    anchor=north,legend columns=1},    symbolic x coords={strict,relaxed, strict$@$5, relaxed$@$5},
    xtick=data,
    ]
\addplot[black,fill=yellow,pattern=north east lines] coordinates {(relaxed$@$5,6.15) (strict$@$5, 1.86)};
\addplot[olive,fill=olive] coordinates {(relaxed$@$5,0.92) (strict$@$5,0.85)};
\addplot[teal,fill=teal] coordinates {(relaxed$@$5,3.64) (strict$@$5,1.03)};
\addplot[black,fill=blue!25!white] coordinates {(relaxed$@$5,11.70) (strict$@$5,8.38)};
\addplot[black,fill=blue!75!black] coordinates {(relaxed$@$5,12.69) (strict$@$5,6.08)};
\legend{ConceptNet,WebChild,TupleKB,Q'modo-$\tau$, Q'modo-$\sigma$}
\end{axis}
\end{tikzpicture}

==> parts/csk.tex <==
\section{Common Sense Knowledge}

\jr{I am just writing down some ideas which can be useful for the future.}

A definition of common sense knowledge fails to win unanimous support. Some prefer a pragmatic approach, considering that a common knowledge refers to something all humans know. However, knowledge is dynamic and depends on people and culture. So, it evolves during the life of a person and a society. Let us quote some examples of variability: 
\begin{itemize}
    \item it might be trivial now that Earth is a sphere, it was not always the case.
    \item a french boy knows what is a chocolatine, but it is very unlikely a American one can say what it is.
    \item Pythagoras formula is trivial for a high school student in the U.S. but it magic to an average 8-years old child.
    \item Maxwell equations are common knowledge for a physicist but are unknown by most of the population
\end{itemize}

To fix these variation, some people fix a common state which occurred to many individuals and which present few variability inside a group. For example, one could define commonsense knowledge as a knowledge an average 8 years old child living in the U.S. would know. The hope is to create a reference person who only knows things he observed, both from the physical and social world.
This kind of definition was used in TupleKB~\cite{tuplekb}, in which they fix the age and the domain (although TupleKB does not claim to do exactly common sense knowledge). However, even if we skip the question of the existence of such an individual, this definition makes the discovery and validation of the facts quite a challenge: getting data from children creates both an ethical and practical problem. In TupleKB, textbooks are used to evaluate the performances of the system but in general, common sense is rarely taught.

Instead of directly tackle the definition of commonsense knowledge, we could try to define what are the required properties of such a knowledge. We consider the following list:

\begin{itemize}
    \item \textbf{Universality}: the knowledge is shared by almost all individuals of a group. So, the knowledge (chocolatine, contains, chocolate) is commonsense as it is shared by almost all French.
    \item \textbf{Meaningfulness}: one could imagine a situation in which the knowledge is true, even if it is absurd. For example, (zebra, eat, lion) is meaningful, although the situation is very unlikely to happen. On the other hand, (mouse, eat, eat) does not make sense.
    \item \textbf{Typicality}: one can evaluate if a fact is likely to happen or not. For example, (zebra, eat, lion) has a low typicality and ($E$, equals, $mc^2$) is certain. A low typicality can also be considered commonsense but it should be mentionned. For example, people know meteorites often enter the atmosphere but they also know it is very unlikely to get hit by one.
    \item \textbf{Discriminability}: the knowledge is a distinctive feature. For example, (zebra, has, cell) does not discriminate much the zebras whereas (zebra, has, white and black stripes) is more specific. This discriminability can be linked to unexpectedness and the simplicity theory which are used in cognitive science (references ?) and is in general hard to evaluate.
    \item \textbf{Generality}: the set of commonsense knowledge covers a broad specter of topics. In general, humans do not have only domain specific knowledge.
\end{itemize}

If we look at previous work, we can notice that most commonsense knowledge base focus on specific aspects.
Webchild evalutation is done mainly on meaningfulness. However, as it is based on very contextualized data (the Google N-grams), the universality, typicality and discriminability are in general very low (should we include our initial analysis or just a future Turk evaluation ?)


==> parts/intro-old.tex <==
\section{Introduction}

\subsection{Motivation}

Common-sense knowledge and reasoning is an old dream of the AI field, already envisioned by McCarthy in the 1960s~\cite{mccarthy1960programs}. Common sense knowledge includes basic assertions like \emph{(monkeys, like, bananas)}, \emph{(rain, causes, wet ground)}, or \emph{(climate change, threatens, biodiversity)}. Such knowledge is a fundamental asset for applications such as question answering, dialogue systems, or reasoning and planning. This holds especially in the face of recent trends towards large-scale end-to-end learning, which yields impressive results on selected tasks, but greatly limits the ability to reuse and generalize learned models.

Collecting and structuring common-sense knowledge is difficult for several reasons: The nature of common-sense is that it is often implicitly known by humans, but hardly expressed in structured or semi-structured form, thus making automated extraction difficult. Similarly, it is very difficult to establish a notion of salience on common-sense, i.e., to determine what are relevant and/or interesting statements about a given subject.

Several works have targeted the construction of large common-sense knowledge bases in the past. An early approach is the CYC project, which had experts write down common-sense assertions and rules~\cite{lenat1995cyc}. Another prominent approach, ConceptNet, used crowdsourcing for better scalability~\cite{conceptnet}. Since then, various projects have focused on automatic common-sense knowledge base (CSKB) construction from text and image sources, most prominently WebChild~\cite{webchild} and TupleKB~\cite{tuplekb}.  

These efforts have produced encouraging initial repositories of common-sense assertions. Nevertheless, they exhibit important limitations, in particular w.r.t.\ their generality, relevance, size, and informativeness of predicates.

\subsection{Approach and Contributions}

In this paper we present QUASIMODO, a framework for automated large-scale CSKB construction. Our framework utilizes targeted novel sources for information extraction, affirmative questions from search engine query logs and discussion and question-answering forums. In a recall-oriented extraction stage, it utilizes customized open information extraction to extract candidate triples. These triples are normalized in several carefully crafted steps, then fed into a precision-oriented validation stage, where frequency information across sources, along with linguistic cues and frequencies in search engine snippets are used to estimate typicality and correctness.

The superiority of this pipeline w.r.t.\ ConceptNet, WebChild and TupleKB is evaluated along a set of dimensions, covering the intrinsic metrics of size, correctness, typicality and ranking ability, and extrinsic evaluations in textbook coverage, question answering and Taboo forbidden term prediction.


\paragraph{Contributions}
Our approach, Q2CSK provides the following salient and original contributions:
\begin{enumerate}
    \item A principled multi-source 3-stage extraction-normalization-validation methodology, along with a sample instantiation that yields knowledge of significantly higher coverage and precision than existing sources; 
    \item The exploitation of affirmative question sources, allowing to extract knowledge that would hardly be present explicitly anywhere else;
    \item A dataset of 1.5 million common-sense assertions for 13,000 concepts, which outperforms state-of-the-art CSKBs by at least ZYX\% in intrinsic preference and YXZ\% in coverage, and YXZ\% in extrinsic use cases of science question answering and ZXY\% for summarization.
\end{enumerate}

TODO: Say somewhere that we tap Google's knowledge 3 times - search logs, index (snippets), and co-occurrence (n-grams).

==> parts/notes.tex <==
\appendix

\section{Todo}

\begin{enumerate}
    \item porcupine teeth are white, porcupine, are white, teeth $->$ what should we do about these results?
    \item Why do we beat ConceptNet extrinsically, but not intrinsically? This needs an explanation, otherwise will raise questions.
\end{enumerate}

\section{Notes}

\begin{enumerate}
    \item 9+1 pages
    \item If more extrinsic evaluations are needed then see tasks where embeddings were evaluated (w2vec competitors).
    \item Evaluation via some word-word relatedness benchmarks (ACL 2015 overview paper?)
    \item Evaluation via summary generation (triple-to-sequence models).
    \item Ranking: Typical things should be common in images, but rare in news. So we might get frequencies from image search (Flickr/Pinterest?), and compare with frequencies on Google News (and various other frequencies). Challenge: Google image search does not give hit counts.
    \item Tuning of our results as advantage - with scores - ConceptNet cannot do that
    \item Subsubsection(Crowdsourced preference) - Wile the precision/recall evaluations indirectly compare across KBs (how correct/typical is each KB, how much does it cover), we could more directly compare KBs by taking top-k facts for specific subjects, and asking for preference among pairs next to each other.
    \item Extrinsic evaluation wrt.\ Britannica Kids was removed
    \item possible inconsistency: koninika clustering results is on new predicates from archit, which we now do not use anymore
    \item antonym checking can still put it, even if not significant...
    \item Case study: show top 5 facts? would be more resilient, than handpicked samples
    \item Precision evaluation best for 3 datasets: 1) all triples, 2) sampled according to confidence, 3) top 5 per subject in each vertical
    \item Book n-grams are not used, or?
    \item How to output clustering on dropbox?
    \item How to formalize modalities, negation?
\end{enumerate}

\section{Planned page distribution}

1 Intro  		1.5

2 Related work	0.5

3 System		0.5

4 Qlogs+forums	1

5 Snippets		1

6 Cleaning+fusion 1

7 Grouping		1

8 Experiments	2

9 0.25

= 8.75

==> parts/qa_explanation_normal.tex <==
\noindent{\bf Answer Selection for QA.}
In this use case, we show that CSK helps in selecting answers
for multiple-choice questions. We use five datasets: (i+ii) elementary school and middle school science questions from the AllenAI science challenge~\cite{ai2-dataset}, (iii) commonsense questions generated from ConceptNet~\cite{commonsenseqa}, (iv) reading comprehension questions from the TriviaQA dataset~\cite{triviaqa}, and (v) exam questions from the Indian exam training platform Examveda~\cite{parchureveda}. The baseline are given by AllenAI, in aristo-mini\footnote{https://github.com/allenai/aristo-mini}.

To assess the contribution of CSKBs, for each multiple-choice answer
and each word t in the answer phrase, 
we look for all triples of the form (t, p, o) or (s, p, t) in a KB;
each time s or o appears in the respective question, 
we increase the score of that answer. 
In the end, the answer with the highest score is chosen (or 
the lexicographic first if two answers have equal scores).
%$\geq1$).
As there might be no relevant triples for a question, the algorithm
can decided to not answer. So, we also report the recall.
This is a basic strategy for multiple-choice QA and could
 be improved in many ways. However, it is sufficient to
bring out the value of CSK and the differences between the CSKBs under test.

We compare four CSKBs against each other and
against a word2vec baseline which computes the embeddings
similarity between questions and answers.
%in order to assess where the common-sense facts add more than just association knowledge.
The results are shown in Table~\ref{tbl:QA}. 
%As one can see, 
Quasimodo significantly outperforms the other CSKBs on three of the five datasets
and is competitive on the other two.

==> parts/qa_results_normal.tex <==
\begin{table*}
    \centering
    \scalebox{0.9}{
    \begin{tabular}{cccccc}
        \hline
        KB & Elementary NDMC & Middle NDMC & CommonsenseQA & Trivia & Examveda \\
        \hline
        \#Questions & 1,288 & 1,409 & 7,609 & 452 & 765 \\ \hline
        Random & 27.1/27.1 & 24.6/24.6 & 33.6/33.6 & 25.9/25.9 & 25.4/25.4 \\
        word2vec & 28.6/27.7 & 28.3/26.6 & 39.3/38.5 & 28.3/23.2 & 27.2/22.1 \\
%        ElasticSearch & 45/45 & 41.8/41.8 & 38.2/38.2 & 31.6/31.6 & 37.9/37.9 \\ 
\hdashline
        Quasimodo & \textbf{38.0*}/\textbf{37.3*} & \textbf{37.4*}/\textbf{35.9*} & \textbf{38.4*}/\textbf{36.1*} & 30.4/\textbf{22.7*} & \textbf{32.8}/\textbf{21.3*} \\
        ConceptNet & 32.5/21.4 & 25.9/14.6 & - (source) & \textbf{32.1}/7.74 & 29.8/5.88 \\
        TupleKB & 32.6/25 & 30.6/22.2 & 37.2/17.5 & 23.1/3.3 & 31.6/4.71 \\
        WebChild & 24.8/21.1 & 28.9/24.3 & 31.1/26.3 & 27.6/10.6 & 25.5/8.24 \\
    \hline
    \end{tabular}
    }
    \caption{Precision and recall of answer selection in question answering. Statistically significant results (with p-value $< 0.05$ for paired t-test) of Quasimodo against other CSKBs are marked with an asterisk.}
    \label{tbl:QA}
    \vspace{-0.6cm}
\end{table*}
% 38.0/33.3 scores of conceptnet on commonsenseQA

==> parts/snippets.tex <==
\section{Candidate Gathering from Search Engine Answer Snippets}

\sr{Archit: We are also using the titles, right? Do they play a reasonable role? If yes I will emphasize them, to press the point that grammar-reliant OpenIE does not work}

\as{We are also using titles as they also are a good source for predicates. Titles are mostly single sentences, many times incomplete, ungrammatical but a bit more relaxed than snippets. We can make our case that our model generalizes to both complex, contextless text like the snippets and also to something moderate, simpler to understand text like the titles}

To overcome sparseness and reporting bias w.r.t.\ common sense assertions, it is desirable to tap text resources as large as possible, with the largest possible corpus being the whole web. WebChild and TupleKB followed a similar rationale, with WebChild tapping fragments by using the Google Web 1T N-Gram dataset, and TupleKB by running OpenIE on top-10 results of instantiations of crafted domain-specific Bing queries like ``[animal\_name] adaption environment''.

We follow a similar rationale as TupleKB, accessing the web via search queries, however without the limitation of manually crafting queries.

To overcome the sparsity of signals in web search results, we perform targeted queries with subject-object candidates, looking for specific predicates linking them. Given for instance a suspected relationship between \fact{landlord} and \fact{deposit}, we query search engines with the search phrase ``landlord deposit'', in order to find relevant predicates. While this targeted search lowers recall, it allows a significantly higher precision, as snippets are likely relevant to the specific S-O-pair, thus increasing desirable statistical redundancy.

\paragraph{Predicate identification}
TupleKB relied on OpenIE for extracting information from snippets. Our analysis showed that OpenIE results on snippets are often of low quality and miss important predicates because OpenIE relies on 1) correct grammar, 2) complete sentences, and 3) only discovers predicates within single sentences. These conditions are often violated in snippets, where snippets may contain ungrammatical title phrases, contain only parts of sentences with ellipses, or convey important information across sentence borders.

\sr{Examples?}
\as{This seems like a good example as there are 3 separate nonconsecutive texts: "I dont know why ppl are making a fuss about the baby zebra....Its the wild .... Stupid King Lion, he could hunt ... "}

We, therefore, build our own supervised classifier for predicting whether verb phrases in a snippet represent predicates for given S-O-pairs.

Given verb phrases identified via a regular expression on part-of-speech tags, we build feature vectors capture syntactic information, in particular the distance w.r.t.\ occurrences of S and O in the snippet, and the POS tags of surrounding tokens, and semantic information, in particular the word2vec average, maximum and minimum similarity between tokens in the verb phrase and S and O and surrounding tokens.

\paragraph{Training}

We train the classifier using 500 simple triples from the \fact{isCapableOf} relation of ConceptNet. For each of these, we generate 50 search snippets by querying for S, P and O together \sr{True? Or do we only query for S and O?}\as{Yes, for training only SPO. For testing we use SO}, then label each occurrence of P in the snippets as a positive training example, each other predicate as a negative example. Overall, this gives 43k positive examples, and 248k negative examples. \sr{Archit: Please check numbers} \as{The numbers changed slightly since I lemmatized and combined them. The original examples were 38K positive and 195K negative examples, but with the constraint that snippets must include SO, this number comes down to 15K positive and 67K negative examples. }
On withheld data, the classifier achieves 74.8\% precision and 73.8\% recall. 

\paragraph{Aggregation}

Although precision and recall still leave room for improvement, in combination with frequency observations, they allow solid insights into relevant predicates.
For instance, for the S-O-pair \fact{landlord} and \fact{rent}, Google our classifier on the top 50 Google snippets 16 times predicts the predicate \fact{refund}, 12 times \fact{deduct from}, and 6 times \fact{put}.

To increase the resilience of the approach, we not only query one search engine but 5 complimentary ones: Google, Youtube, Flickr, Istockphoto and Pinterest, thus obtaining several frequencies that can be used in the following cleaning and refinement phases.

\sr{TODO: Talk about cost, scalability} 
